LinGBM: A Performance Benchmark for Approaches to Build GraphQL Servers (Extended Version)

GraphQL is a popular new approach to build Web APIs that enable clients to retrieve exactly the data they need. Given the growing number of tools and techniques for building GraphQL servers, there is an increasing need for comparing how particular approaches or techniques affect the performance of a GraphQL server. To this end, we present LinGBM, a GraphQL performance benchmark to experimentally study the performance achieved by various approaches for creating a GraphQL server. In this article, we discuss the design considerations of the benchmark, describe its main components (data schema; query templates; performance metrics), and analyze the benchmark in terms of statistical properties that are relevant for defining concrete experiments. Thereafter, we present experimental results obtained by applying the benchmark in three different use cases, which demonstrates the broad applicability of LinGBM.

==> Application4.tex <==
%\subsection{Use 'out-of-the-box' tools together with schema delegation} \label{sec:Use-'out-of-the-box-schema-delegation}
\subsection{Schema Delegation} \label{subsec:UC4}

%\subsubsection{set up the experiment}
%~\\
As mentioned in Section~\ref{sec:Hand-coding-resolver}, the auto-generated GraphQL schema by such tools like 
Hasura and PostGraphQL may be different from the designed GraphQL schema. Schema delegation can be used to create a mapping between the auto-generated schema and the customized schema. In this section, we take Hasura as an example and observe how the schema delegation affects the performance of the GraphQL server.

%\subsubsection{Results and Discussion of the Experiment}

We are interested to know how much impact of using schema delegation over Hasura comparing with pure Hasura. Observing Figure~\ref{Fig:G_H_tp_client}
, it is not surprising to find that pure Hasura works better than Hasura with delegation. H+D can handle much fewer queries within the same time period. To get a better understanding of the effect of schema delegation, more research on the implementation of scheme delegation is needed. However, we would like to keep this as further work as it is not the main aim of this paper.

% Show some removed Figures:
%\input{ThroughputResult}
%\input{QETResult}

==> QETResult.tex <==
%1. 
% QETt, 
% Naive, B, C, B+C
% 1 client, all QTs
\begin{figure*}[ht]
  \centering
  \subfloat[QT1]{\label{figur:QT1}\includegraphics[width=0.12\linewidth]{figure/QET_QT_v3/QT1.png}}%
  \subfloat[QT2]{\label{figur:QT2}\includegraphics[width=0.12\linewidth]{figure/QET_QT_v3/QT2.png}}%
  \subfloat[QT3]{\label{figur:QT3}\includegraphics[width=0.12\linewidth]{figure/QET_QT_v3/QT3.png}}%
  \subfloat[QT4]{\label{figur:QT4}\includegraphics[width=0.12\linewidth]{figure/QET_QT_v3/QT4.png}}%
  %\\
  \subfloat[QT5]{\label{figur:QT5}\includegraphics[width=0.12\linewidth]{figure/QET_QT_v3/QT5.png}}%
  \subfloat[QT6]{\label{figur:QT6}\includegraphics[width=0.12\linewidth]{figure/QET_QT_v3/QT6.png}}%
  \subfloat[QT7]{\label{figur:QT7}\includegraphics[width=0.12\linewidth]{figure/QET_QT_v3/QT7.png}}%
  \subfloat[QT8]{\label{figur:QT8}\includegraphics[width=0.12\linewidth]{figure/QET_QT_v3/QT8.png}}%
  \\
  \subfloat[QT9]{\label{figur:QT9}\includegraphics[width=0.12\linewidth]{figure/QET_QT_v3/QT9.png}}%
  \subfloat[QT10]{\label{figur:QT10}\includegraphics[width=0.12\linewidth]{figure/QET_QT_v3/QT10.png}}%
  \subfloat[QT11]{\label{figur:QT11}\includegraphics[width=0.12\linewidth]{figure/QET_QT_v3/QT11.png}}%
  \subfloat[QT12]{\label{figur:QT12}\includegraphics[width=0.12\linewidth]{figure/QET_QT_v3/QT12.png}}%
  %\\
  \subfloat[QT13]{\label{figur:QT13}\includegraphics[width=0.12\linewidth]{figure/QET_QT_v3/QT13.png}}%
  \subfloat[QT14]{\label{figur:QT14}\includegraphics[width=0.12\linewidth]{figure/QET_QT_v3/QT14.png}}%
  \subfloat[QT15]{\label{figur:QT15}\includegraphics[width=0.12\linewidth]{figure/QET_QT_v3/QT15.png}}%
  \subfloat[QT16]{\label{figur:QT16}\includegraphics[width=0.12\linewidth]{figure/QET_QT_v3/QT16.png}}%
  \caption{QETt of each template on different GraphQL servers}
  \label{Fig:QETperQTonDiffServer}
  \Description{}
\end{figure*}


% QET1
% Naive, Hasura, Postgraphile
% 1 client, db10, db15, db20
\begin{figure*}[ht]
  \centering
  \subfloat[Naive]{\label{Fig:QETq_datasetSize_Naive}\includegraphics[width=\linewidth]{figure/QET_q/Naive_db10_15_20_log.png}}%
  \\
  \subfloat[Postgraphile]{\label{Fig:QETq_datasetSize_P}\includegraphics[width=\linewidth]{figure/QET_q/P_db10_15_20_log.png}}%
  \\
  \subfloat[Hasura]{\label{Fig:QETq_datasetSize_H}\includegraphics[width=\linewidth]{figure/QET_q/H_db10_15_20_log.png}}%
  \caption{Query Execution time (aQETq) of single queries on different datasets}
  \label{Fig:QETq_datasetSize}
  \Description{}
\end{figure*}





==> QueryStatsTables.tex <==
\begin{table}[t]
\centering
%\caption{}
%\inlinetodo{Sijin: Done. Add captions to the sub-tables}
	%\small
	\fontsize{7}{8} \selectfont
%\begin{minipage}{.55\linewidth}
%\caption{Number of query instances of each query template~\\at different scale factors ($\sfactor$).}
\caption{Query instances\#}
\label{tab:Scale-NumberOfInstance-QT}
\vspace{-4mm} % Layout Adjustment
\begin{tabular}{@{}c|rrrrr}
\hline
& $\sfactor=1$ & $\sfactor=5$ & $\sfactor=10$ & $\sfactor=15$ & $\sfactor=20$ \\ \hline
QT1 & 540 & 3,373 & 6,843 & 10,521 & 14,457 \\
QT2 & 1,000 & 1,000 & 1,000 & 1,000 & 1,000 \\
QT3 & 224 & 1,371 & 2,827 & 4,407 & 6,032 \\
QT4 & 93 & 562 & 1,128 & 1,745 & 2,399 \\
QT5 & 15 & 93 & 189 & 293 & 402 \\
QT6 & 1,000 & 1,000 & 1,000 & 1,000 & 1,000 \\
QT7 & 48,950 & 246,500 & 493,250 & 740,400 & 989,250 \\
QT8 & 15,000 & 15,000 & 15,000 & 15,000 & 15,000 \\
QT9 & 2,000 & 2,000 & 2,000 & 2,000 & 2,000 \\
QT10 & 27,077 & 170,576 & 344,750 & 530,133 & 728,208 \\
QT11 & 1,000 & 1,000 & 1,000 & 1,000 & 1,000 \\
QT12 & 14,685 & 458,490 & 1,864,485 & 4,338,744 & 7,953,570 \\
QT13 & 899,701 & 27,893,940 & 113,921,020 & 262,560,648 & 480,241,305 \\
QT14 & 6,297,907 & 195,257,580 & 797,447,140 & 1,837,924,536 & 3,361,689,135 \\
QT15 & 1,000 & 1,000 & 1,000 & 1,000 & 1,000 \\
QT16 & 1,000 & 1,000 & 1,000 & 1,000 & 1,000
\\ \hline
\end{tabular}
%\end{minipage}%
% 
% \begin{minipage}{.19\linewidth}
% \caption{Leaf nodes\#}
% \label{tab:estimated-no-of-leaf-nodes}
% \begin{tabular}{@{}c|rr|rr|rr}
% & min & max & \multicolumn{2}{|l|}{avg.\ at $\sfactor$=10} & \multicolumn{2}{l}{avg.\ at $\sfactor$=20} \\ \hline
% QT1 & 0 & 7$\cdot\sfactor$ & 25 & ($\pm$4.44) & 54 & ($\pm$3.44) \\
% QT2 & 0 & 80$\cdot\sfactor$ & 91 & ($\pm$35.419 & 163 & ($\pm$51.44) \\
% QT3 & 1 & 1 & 1 & ($\pm$0.00) & 1 & ($\pm$0.00) \\
% QT4 & 0 & 7$\cdot\sfactor$ & 27 & ($\pm$4.40) & 54 & ($\pm$6.99) \\
% QT5 & 0 & 49$\cdot\sfactor^2$ & 875 & ($\pm$60.84) & 1813 & ($\pm$114.63) \\
% QT6 & 0 & 7$\cdot\sfactor$ & 25 & ($\pm$5.13) & 51 & ($\pm$7.72) \\
% QT7 & 0 & 10 & 3 & ($\pm$4.32) & 9 & ($\pm$2.18) \\
% QT8 & 500 & 1000 & 772 & ($\pm$131.07) & 774 & ($\pm$138.74) \\
% QT9 & 0 & 140$\cdot\sfactor$ & 311 & ($\pm$60.85) & 629 & ($\pm$54.11) \\
% QT10 & 0 & 6300$\cdot\sfactor$ & 6 & ($\pm$4.47) & 13 & ($\pm$8.41) \\
% QT11 & 0 & 7$\cdot\sfactor$ & 24 & ($\pm$4.73) & 51 & ($\pm$5.81) \\
% QT12 & 0 & 840 & 14 & ($\pm$6.85) & 17 & ($\pm$4.99) \\
% QT13 & 0 & 21$\cdot\sfactor$ & 0 & ($\pm$0.00) & 0 & ($\pm$0.00) \\
% QT14 & 0 & 21$\cdot\sfactor$ & 0 & ($\pm$0.00) & 0 & ($\pm$0.00) \\
% QT15 & 1 & 1 & 1 & ($\pm$0.00) & 1 & ($\pm$0.00) \\
% QT16 & 1 & 1 & 1 & ($\pm$0.00) & 1 & ($\pm$0.00)
% \end{tabular}
% \end{minipage}
% 
%\begin{minipage}{.24\linewidth}
%\caption{Type of duplicate ~\\in results of each query template.}
%\caption{Type of duplicate}
%\label{tab:duplicate-metrics}
%\begin{tabular}{@{}c|cccc}
%& LLD & ILD & ND & DF \\ \hline
%QT1 &  &  &  & X \\
%QT2 &  & &  & X\\
%QT3 &  &  &  & X \\
%QT4 &  &  & (X) & \\
%QT5 &  &  & X &  \\
%QT6 &  &  & (X) & \\
%QT7 & (X) &  &  & \\
%QT8 &  &  &  & X \\
%QT9 &  & (X) &  & \\
%QT10 &  &  &  & X \\
%QT11 &  &  &  & X\\
%QT12 &  &  &  & X\\
%QT13 & (X) &  &  & \\
%QT14 & (X) &  &  & \\
%QT15 &  &  &  & X \\
%QT16 &  &  &  & X
%\end{tabular}
%\end{minipage}
\end{table}



% \begin{table}[t]
% \centering
% \small
% \caption{Leaf nodes\#}%
% \label{tab:estimated-no-of-leaf-nodes}%
% \begin{minipage}{.47\linewidth}
% \centering
% \vspace{-4mm} % Layout Adjustment
% \begin{tabular}{@{}c|rr}
% \hline
% & min & max \\ \hline
% QT1 & 0 & 7$\cdot\sfactor$  \\
% QT2 & 0 & 80$\cdot\sfactor$ \\
% QT3 & 1 & 1 \\
% QT4 & 0 & 7$\cdot\sfactor$ \\
% QT5 & 0 & 49$\cdot\sfactor^2$ \\
% QT6 & 0 & 7$\cdot\sfactor$ \\
% QT7 & 0 & 10 \\
% QT8 & 500 & 1000 \\
% \hline
% \end{tabular}
% \end{minipage}
% \quad
% \begin{minipage}{.47\linewidth}
% \centering
% \vspace{-4mm} % Layout Adjustment
% \begin{tabular}{@{}c|rr}
% \hline
% & min & max \\ \hline
% QT9 & 0 & 1000 \\
% QT10 & 0 & 6300$\cdot\sfactor$ \\
% QT11 & 0 & 7$\cdot\sfactor$ \\
% QT12 & 0 & 840 \\
% QT13 & 0 & 21$\cdot\sfactor$ \\
% QT14 & 0 & 21$\cdot\sfactor$ \\
% QT15 & 1 & 1 \\
% QT16 & 1 & 1 \\
% \hline
% \end{tabular}
% \end{minipage}
% \end{table}


\begin{table}[t]
    \centering
		%\small
		\fontsize{7}{8} \selectfont
    \caption{Leaf nodes\#}%
    \label{tab:estimated-no-of-leaf-nodes}%
    \vspace{-4mm} % Layout Adjustment
    \begin{tabular}{c|cccccccc}
        \hline
                              & QT1              & QT2                 & QT3              & QT4              & QT5                 & QT6               & QT7  & QT8  \\ \hline
        min                   & 0                & 0                   & 1                & 0                & 0                   & 0                 & 0    & 500  \\
        max                   & 7$\cdot\sfactor$ & 80$\cdot\sfactor$   & 1                & 7$\cdot\sfactor$ & 49$\cdot\sfactor^2$ & 7$\cdot\sfactor$  & 10   & 1000 \\ \hhline{=========}
                              & QT9              & QT10                & QT11             & QT12             & QT13                & QT14              & QT15 & QT16 \\ \hline
        min                   & 0                & 0                   & 0                & 0                & 0                   & 0                 & 1    & 1    \\
        max                   & 1000             & 6300$\cdot\sfactor$ & 7$\cdot\sfactor$ & 840              & 21$\cdot\sfactor$   & 21$\cdot\sfactor$ & 1    & 1    \\ \hline
        \end{tabular}
\end{table}

==> ThroughputResult.tex <==
%1. 
% database statistics: #queries of each client, #connections #tuple fetched #$tuple returned
% 1 clients, QT5, QT9
\begin{table*}[ht] 
\centering
\captionof{figure}{Throughput at different number of clients (TODO: caption)} 
\label{Tab:pg_stat_database}
\begin{tabular}{p{0.2cm}cccc} 
  & throughput & $\#$total queries & QETt (TP) & $\#$queries of each client \\
  QT5 &
  \includegraphics[width=0.17\linewidth]{figure/tp_NBC_v2/c1_included/QT5.png}%
  &
  \includegraphics[width=0.17\linewidth]{figure/tp_NBC_v2/c1_included/totalSend_QT5.png}%
  &
  % Show the range of query execution time during throughput test (some QETs is up to 60s)
  \includegraphics[width=0.19\linewidth]{figure/tp_NBC_v2/c1_included/QETduringTPtest_QT5.png}
  &
  \\
  QT9
  &
  \includegraphics[width=0.17\linewidth]{figure/tp_NBC_v2/c1_included/QT9.png}%
  &
  \includegraphics[width=0.17\linewidth]{figure/tp_NBC_v2/c1_included/totalSend_QT9.png}%
  &
  \includegraphics[width=0.19\linewidth]{figure/tp_NBC_v2/c1_included/QETduringTPtest_QT9.png}
  &
  \\
  &QETt(c1) & $\#$connections & $\#$tuple fetched & $\#$tuple returned\\
  QT5
  &
  \includegraphics[width=0.15\linewidth]{figure/QET_QT_v3/QT5.png}%
  &
  \includegraphics[width=0.15\linewidth]{figure/db_statics/connectedBackend/QT5.png}%
  &
  \includegraphics[width=0.15\linewidth]{figure/db_statics/tup_fetched/QT5.png}%
  &
  \includegraphics[width=0.15\linewidth]{figure/db_statics/tup_returned/QT5.png}%
  \\
  QT9
  &
  \includegraphics[width=0.15\linewidth]{figure/QET_QT_v3/QT9.png}%
  &
  \includegraphics[width=0.15\linewidth]{figure/db_statics/connectedBackend/QT9.png}%
  &
  \includegraphics[width=0.15\linewidth]{figure/db_statics/tup_fetched/QT9.png}%
  &
  \includegraphics[width=0.15\linewidth]{figure/db_statics/tup_returned/QT9.png}%
\end{tabular}
\end{table*}


% 2.
% throughput
% #client: 1, 250, 500, 750, 1000
% Naive, B, C, B+C
% all QTs
\begin{figure*}[ht]
  \centering
  \subfloat[QT1]{\label{figur:tp_QT1}\includegraphics[width=0.25\linewidth]{figure/tp_NBC_v2/c1_included/QT1.png}}%
  \subfloat[QT2]{\label{figur:tp_QT2}\includegraphics[width=0.25\linewidth]{figure/tp_NBC_v2/c1_included/QT2.png}}%
  \subfloat[QT3]{\label{figur:tp_QT3}\includegraphics[width=0.25\linewidth]{figure/tp_NBC_v2/c1_included/QT3.png}}%
  \subfloat[QT4]{\label{figur:tp_QT4}\includegraphics[width=0.25\linewidth]{figure/tp_NBC_v2/c1_included/QT4.png}}%
  \\
  \subfloat[QT5]{\label{figur:tp_QT5}\includegraphics[width=0.25\linewidth]{figure/tp_NBC_v2/c1_included/QT5.png}}%
  \subfloat[QT6]{\label{figur:tp_QT6}\includegraphics[width=0.25\linewidth]{figure/tp_NBC_v2/c1_included/QT6.png}}%
  \subfloat[QT7]{\label{figur:tp_QT7}\includegraphics[width=0.25\linewidth]{figure/tp_NBC_v2/c1_included/QT7.png}}%
  \subfloat[QT8]{\label{figur:tp_QT8}\includegraphics[width=0.25\linewidth]{figure/tp_NBC_v2/c1_included/QT8.png}}%
  \\
  \subfloat[QT9]{\label{figur:tp_QT9}\includegraphics[width=0.25\linewidth]{figure/tp_NBC_v2/c1_included/QT9.png}}%
  \subfloat[QT10]{\label{figur:tp_QT10}\includegraphics[width=0.25\linewidth]{figure/tp_NBC_v2/c1_included/QT10.png}}%
  \subfloat[QT11]{\label{figur:tp_QT11}\includegraphics[width=0.25\linewidth]{figure/tp_NBC_v2/c1_included/QT11.png}}%
  \subfloat[QT12]{\label{figur:tp_QT12}\includegraphics[width=0.25\linewidth]{figure/tp_NBC_v2/c1_included/QT12.png}}%
  \\
  \subfloat[QT13]{\label{figur:tp_QT13}\includegraphics[width=0.25\linewidth]{figure/tp_NBC_v2/c1_included/QT13.png}}%
  \subfloat[QT14]{\label{figur:tp_QT14}\includegraphics[width=0.25\linewidth]{figure/tp_NBC_v2/c1_included/QT14.png}}%
  \subfloat[QT15]{\label{figur:tp_QT15}\includegraphics[width=0.25\linewidth]{figure/tp_NBC_v2/c1_included/QT15.png}}%
  \subfloat[QT16]{\label{figur:tp_QT16}\includegraphics[width=0.25\linewidth]{figure/tp_NBC_v2/c1_included/QT16.png}}%
  \caption{Throughput accross number of client on different GraphQL servers (C250, C500, C750, C1000)}
  \label{Fig:TP_perQT}
  \Description{}
\end{figure*}



% 2.
% throughput
% #client: 1, 250, 500, 750, 1000
% Hasura, PostGraphile, H+delegation
% all QTs
\begin{figure*}[ht]
  \centering
  \subfloat[QT1]{\label{figur:G_H_tp_QT1}\includegraphics[width=0.12\linewidth]{figure/tp_PHD_v2/c1_included/QT1.png}}%
  \subfloat[QT2]{\label{figur:G_H_tp_QT2}\includegraphics[width=0.12\linewidth]{figure/tp_PHD_v2/c1_included/QT2.png}}%
  \subfloat[QT3]{\label{figur:G_H_tp_QT3}\includegraphics[width=0.12\linewidth]{figure/tp_PHD_v2/c1_included/QT3.png}}%
  \subfloat[QT4]{\label{figur:G_H_tp_QT4}\includegraphics[width=0.12\linewidth]{figure/tp_PHD_v2/c1_included/QT4.png}}%
  %\\
  \subfloat[QT5]{\label{figur:G_H_tp_QT5}\includegraphics[width=0.12\linewidth]{figure/tp_PHD_v2/c1_included/QT5.png}}%
  \subfloat[QT6]{\label{figur:G_H_tp_QT6}\includegraphics[width=0.12\linewidth]{figure/tp_PHD_v2/c1_included/QT6.png}}%
  \subfloat[QT7]{\label{figur:G_H_tp_QT7}\includegraphics[width=0.12\linewidth]{figure/tp_PHD_v2/c1_included/QT7.png}}%
  \subfloat[QT8]{\label{figur:G_H_tp_QT8}\includegraphics[width=0.12\linewidth]{figure/tp_PHD_v2/c1_included/QT8.png}}%
  \\
  \subfloat[QT9]{\label{figur:G_H_tp_QT9}\includegraphics[width=0.12\linewidth]{figure/tp_PHD_v2/c1_included/QT9.png}}%
  \subfloat[QT10]{\label{figur:G_H_tp_QT10}\includegraphics[width=0.12\linewidth]{figure/tp_PHD_v2/c1_included/QT10.png}}%
  \subfloat[QT11]{\label{figur:G_H_tp_QT11}\includegraphics[width=0.12\linewidth]{figure/tp_PHD_v2/c1_included/QT11.png}}%
  \subfloat[QT12]{\label{figur:G_H_tp_QT12}\includegraphics[width=0.12\linewidth]{figure/tp_PHD_v2/c1_included/QT12.png}}%
  %\\
  \subfloat[QT13]{\label{figur:G_H_tp_QT13}\includegraphics[width=0.12\linewidth]{figure/tp_PHD_v2/c1_included/QT13.png}}%
  \subfloat[QT14]{\label{figur:G_H_tp_QT14}\includegraphics[width=0.12\linewidth]{figure/tp_PHD_v2/c1_included/QT14.png}}%
  \subfloat[QT15]{\label{figur:G_H_tp_QT15}\includegraphics[width=0.12\linewidth]{figure/tp_PHD_v2/c1_included/QT15.png}}%
  \subfloat[QT16]{\label{figur:G_H_tp_QT16}\includegraphics[width=0.12\linewidth]{figure/tp_PHD_v2/c1_included/QT16.png}}%
  \caption{Average throughput (aTPt) accross number of client on different GraphQL servers}
  \label{Fig:postGrap_Hasur_del_TP_perQT}
  \Description{}
\end{figure*}


